Validating an Approach to Formalize Use Cases with Ontologies

Use case driven development methodologies put use cases at the center of the software development process. However, in order to support automated development and analysis, use cases need to be appropriately formalized. This will also help guarantee consistency between requirements specifications and the developed solutions. Formal methods tend to suffer from take up issues, as they are usually hard to accept by industry. In this context, it is relevant not only to produce languages and approaches to support formalization, but also to perform their validation. In previous works we have developed an approach to formalize use cases resorting to ontologies. In this paper we present the validation of one such approach. Through a three stage study, we evaluate the acceptance of the language and supporting tool. The first stage focusses on the acceptance of the process and language, the second on the support the tool provides to the process, and finally the third one on the tool's usability aspects. Results show test subjects found the approach feasible and useful and the tool easy to use.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{J. Kofro\v{n}, J. Tumova, B. Buhnova (Eds.): Formal Engineering\\
Approaches to Software Components and Architectures (FESCA'16)\\
EPTCS 205, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.205.1}{10.4204/EPTCS.205.1}}
\pdfoutput=1

